Multi-line AI-assisted Code Authoring

CodeCompose is an AI-assisted code authoring tool powered by large language models (LLMs) that provides inline suggestions to 10's of thousands of developers at Meta. In this paper, we present how we scaled the product from displaying single-line suggestions to multi-line suggestions. This evolution required us to overcome several unique challenges in improving the usability of these suggestions for developers. First, we discuss how multi-line suggestions can have a 'jarring' effect, as the LLM's suggestions constantly move around the developer's existing code, which would otherwise result in decreased productivity and satisfaction. Second, multi-line suggestions take significantly longer to generate; hence we present several innovative investments we made to reduce the perceived latency for users. These model-hosting optimizations sped up multi-line suggestion latency by 2.5x. Finally, we conduct experiments on 10's of thousands of engineers to understand how multi-line suggestions impact the user experience and contrast this with single-line suggestions. Our experiments reveal that (i) multi-line suggestions account for 42% of total characters accepted (despite only accounting for 16% for displayed suggestions) (ii) multi-line suggestions almost doubled the percentage of keystrokes saved for users from 9% to 17%. Multi-line CodeCompose has been rolled out to all engineers at Meta, and less than 1% of engineers have opted out of multi-line suggestions.

==> RelatedWork_CodeComposePaper.tex <==

%\chandra{I will take another stab once other sections are filled.}
In this section, we review the related work and position our contribution in the literature. 
%
Neural program synthesis is a rapidly evolving area with a large body of work discussing the possibility of applying neural architectures, such as Bayesian networks, and Transformers, to solve program synthesis tasks \cite{bruch2009learning,robles2008program,proksch2015intelligent,zhou22improving, kim21code, chen2021evaluating}. 

%These models are typically evaluated against public data sets such as MBPP (974 Python programming tasks, designed to be solvable by entry-level programmers) \cite{austin2021program} and Human Eval (164 original human-curated Python programming problems) \cite{chen2021evaluating}. The data set we used to evaluate the accuracy of code generation contains 20,000 data points sourced from real code bases, curated across \numLangs programming languages, at \company.

There has been a limited deployment of AI-assisted code generation systems in large-scale industrial environments with tens of programming languages and thousands of developers using them daily \cite{intellicode, codewhisperer, copilot, googleblog}. Availability of research in the public domain is even limited when it comes to evaluating the accuracy of neural program synthesis techniques on large scale industrial data sets and understanding the effects of such tools on software developers using mixed methods studies, 

%\todo{acceptance rates for Copilot 30\%, and we're at 25\%} 

The closest in spirit to our work is the brief blog post from Google \cite{googleblog}. At Google, deploying a hybrid semantic ML code completion to 10k+ Google employees compared to a control group observed a 6\% reduction in coding iteration time (time between builds and tests) when exposed to single-line ML completion. They reported that 3\% of new code (measured in characters) was generated from accepting ML completion suggestions. The acceptance rate for single-line code completions is 25\%. These results demonstrate the impact on developer productivity. In the OSS domain, GitHub CoPilot reported an acceptance rate of 30\% for code completions \cite{GHCP-Acc}.

Our more detailed findings are in line with those found by Google and GitHub with a X\% acceptance rate for \numSuggestionsActivity single-line code completions across \numLangs programming languages. At the same time, our suggestions accounted for X\% of the code written by engineers at \company compared to the X\% reported by Google.

%Further evaluations are necessary to understand the reasons behind ...

There have been a couple of empirical evaluations of GitHub’s Copilot \cite{copilot} in actual use for automatic code completion. Nguyen et al. \cite{nguyen2022empirical} used 33 LeetCode questions to create queries for Copilot in four different programming languages. They found that Copilot's Java suggestions have the highest correctness score (57\%) while JavaScript is the lowest (27\%) \cite{nguyen2022empirical}. While LeetCode examples are useful for algorithmic interview preparation, they differ dramatically from normal engineering work. 

%A study with 15,000 synthetic data points curated from a C\# code base from an industrial software development environment reported an accuracy of 30.7\% for predicting single tokens, such as identifiers, when employing a modified Best Matching Neighbor approach (BMN\#) \cite{8812116}. Offline evaluations of Neural methods for auto-completion in a comparable industrial setting yielded accuracy of 41.9\% on languages with heavily customized frameworks such as Hack \cite{zhou22improving} when tested on a couple of thousands of examples and when tested on open-source data sets (CodeSearchNet) \cite{husain2020codesearchnet} yielded an Exact Match score of 20.10\% and BLEU score of 32.79\% \cite{lu2021codexglue}. Our study of 20,000 data points curated, across \numLangs programming languages, from \company's production code base shows that \cc achieves the highest correctness score of 52\% and BLEU score of 73\% for Hack language and lowest correctness score of 40\% and BLEU score of 56.2\% for C++.

While Copilot is impressive, not all usage of has been positive. A qualitative study  with 24 participants to understand how programmers use and perceive Copilot found that it did not necessarily improve the task completion time or success rate by a significant margin \cite{vaithilingam2022expectation}. However, 19 of 24 participants (79\%) answered that they preferred Copilot over Intellisense. A similar qualitative study of \cc with a larger group of software engineers at \company (70 participants) resulted in a 91.5\% favorable feedback [CITATION NEEDED]. Developers cited reasons such as accelerated coding or typing, helping in discovering new APIs and writing boilerplate code in unknown programming languages, helping with generating documentation for their code, accuracy of suggestions and its ability to predict what the developers are going to type as the main reasons.

\iffalse
An empirical study \cite{peng2023impact} presented a controlled experiment with GitHub Copilot showing recruited software developers who were asked to implement an HTTP server in JavaScript as quickly as possible. The treatment group, with access to Copilot, completed the task 55.8\% faster than the control group. \todo{I'd break this down and address each in wrt \cc}

Amazon's CodeWhisperer \cite{codewhisperer} is a fully functional code completion tool integrated into the IDE. Its analysis found that language models can generate code with correct syntax and pass unit tests in programming languages they are not intentionally trained on. \todo{again, are there metrics we can compare against \cc or technical differences?}
\fi

%\todo{I'd cut this and add some future work, this sounds like an excuse}
%Like the companies discussed above (Google, Microsoft, GitHub, and Amazon), there are several commercial versions of code completion tools by other generative AI companies. The goal here is to provide a sample of the related work rather than undertaking a systematic literature survey of the state of the art. The above works summarize the related work in this area at this point in time in this rapidly changing field.
